Unknotting via null-homologous twists and multi-twists

The untwisting number of a knot K is the minimum number of null-homologous twists required to convert K to the unknot. Such a twist can be viewed as a generalization of a crossing change, since a classical crossing change can be effected by a null-homologous twist on 2 strands. While the unknotting number gives an upper bound on the smooth 4-genus, the untwisting number gives an upper bound on the topological 4-genus. The surgery description number, which allows multiple null-homologous twists in a single twisting region to count as one operation, lies between the topological 4-genus and the untwisting number. We show that the untwisting and surgery description numbers are different for infinitely many knots, though we also find that the untwisting number is at most twice the surgery description number plus 1.

==> commands.tex <==
% Master commands file
% Dependencies: none

\makeatletter
\g@addto@macro\@floatboxreset\centering
\makeatother

\def\mathcenter#1{%
  \vcenter{\hbox{$#1$}}%
}

\allowdisplaybreaks[4]

\addto\extrasamerican{%
  \def\sectionautorefname{Section}%
  \def\subsectionautorefname{Section}%
  \def\subsubsectionautorefname{Section}%
}

\let\fullref\autoref

\newtheorem{theorem}{Theorem}[section]
\newtheorem{conjecture}{Conjecture}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{lemma}{Lemma}[section]

\theoremstyle{definition}
\newtheorem*{convention}{Conventions}
\newtheorem{definition}{Definition}[section]
\newtheorem{example}{Example}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{question}{Question}[section]

\makeatletter
\let\c@conjecture=\c@theorem
\let\c@corollary=\c@theorem
\let\c@proposition=\c@theorem
\let\c@lemma=\c@theorem
\let\c@definition=\c@theorem
\let\c@example=\c@theorem
\let\c@remark=\c@theorem
\let\c@equation\c@theorem
\makeatother

\def\makeautorefname#1#2{\expandafter\def\csname#1autorefname\endcsname{#2}}
\makeautorefname{theorem}{Theorem}%
\makeautorefname{conjecture}{Conjecture}%
\makeautorefname{corollary}{Corollary}%
\makeautorefname{proposition}{Proposition}%
\makeautorefname{lemma}{Lemma}%
\makeautorefname{definition}{Definition}%
\makeautorefname{example}{Example}%
\makeautorefname{remark}{Remark}%
\makeautorefname{question}{Question}

\numberwithin{equation}{section}

\newcommand*{\Alphabet}{ABCDEFGHIJKLMNOPQRSTUVWXYZ1234567890}
\newcommand*{\alphabet}{abcdefghijklmnopqrstuvwxyz1234567890}
\newlength\fcaph
\newlength\fdesc
\newlength\factualfontsize
\settoheight{\fcaph}{\footnotesize \Alphabet}
\settodepth{\fdesc}{\footnotesize \Alphabet \alphabet}
\setlength{\factualfontsize}{\dimexpr\fcaph+\fdesc\relax}

% Comments
\numberwithin{equation}{section}

\newcounter{commentcounter}
\newcommand{\commentb}[1]{\stepcounter{commentcounter}
	\textbf{Comment \arabic{commentcounter} (by B.)}:
	{\textcolor{blue}{#1}} }
\newcommand{\commentm}[1]{\stepcounter{commentcounter}
	\textbf{Comment \arabic{commentcounter} (by M.)}:
	{\textcolor{red}{#1}} }
\newcommand{\commentr}[1]{\stepcounter{commentcounter}
	\textbf{Comment \arabic{commentcounter} (by R.)}:
	{\textcolor{orange}{#1}} }
\newcommand{\comments}[1]{\stepcounter{commentcounter}
	\textbf{Comment \arabic{commentcounter} (by S.)}:
	{\textcolor{BlueGreen}{#1}} }
\newcommand{\commentv}[1]{\stepcounter{commentcounter}
	\textbf{Comment \arabic{commentcounter} (by V.)}:
	{\textcolor{purple}{#1}} }
	
	
\newcommand{\missingref}{\textcolor{orange}{[Ref]}}

% Large / for quotients
\newcommand{\bigslant}[2]{{\raisebox{.2em}{$#1$}\left/\raisebox{-.2em}{$#2$}\right.}}


\newcommand{\TODO}{\textcolor{magenta}{TODO }}

% Text
\newcommand{\OneHalf}{{\textstyle\frac{1}{2}}}
\newcommand{\OneQuart}{{\textstyle\frac{1}{4}}}

% Hyphenation.
\hyphenation{Thurs-ton}
\hyphenation{mo-no-poles}
\hyphenation{sur-ger-y}

%-------------------------------------------------------------------------------

% Pairs of openings and closures
\newcommand{\set}[1]{\mathchoice%
  {\left\lbrace #1 \right\rbrace}%
  {\lbrace #1 \rbrace}%
  {\lbrace #1 \rbrace}%
  {\lbrace #1 \rbrace}%
}
\newcommand{\setc}[2]{\mathchoice%
  {\left\lbrace #1 \, \middle\vert \, #2 \right\rbrace}%
  {\lbrace #1 \, \vert \, #2 \rbrace}%
  {\lbrace #1 \, \vert \, #2 \rbrace}%
  {\lbrace #1 \, \vert \, #2 \rbrace}%
%  {\left\lbrace #1 \, \colon \, #2 \right\rbrace}%
%  {\lbrace #1 \, \colon \, #2 \rbrace}%
%  {\lbrace #1 \, \colon \, #2 \rbrace}%
%  {\lbrace #1 \, \colon \, #2 \rbrace}%
}
\newcommand{\paren}[1]{\mathchoice%
  {\left( #1 \right)}%
  {( #1 )}%
  {( #1 )}%
  {( #1 )}%
}
\newcommand{\brac}[1]{\mathchoice%
  {\left[ #1 \right]}%
  {[ #1 ]}%
  {[ #1 ]}%
  {[ #1 ]}%
}
\newcommand{\abs}[1]{\mathchoice%
  {\left\lvert #1 \right\rvert}%
  {\lvert #1 \rvert}%
  {\lvert #1 \rvert}%
  {\lvert #1 \rvert}%
}
\newcommand{\norm}[1]{\mathchoice%
  {\left\lVert #1 \right\rVert}%
  {\lVert #1 \rVert}%
  {\lVert #1 \rVert}%
  {\lVert #1 \rVert}%
}

% Synonyms for symbols
\newcommand{\eps}{\epsilon}                  % mathord
\newcommand{\veps}{\varepsilon}              % mathord
%\renewcommand{\phi}{\varphi}                 % mathord
\newcommand{\vphi}{\varphi}                  % mathord
\newcommand{\eset}{\varnothing}             % mathord
%\newcommand{\eset}{\emptyset}                % mathord

\newcommand{\dirsum}{\oplus}                 % mathbin
\newcommand{\bigdirsum}{\bigoplus}           % mathop
\newcommand{\tensor}{\otimes}                % mathbin
\newcommand{\bigtensor}{\bigotimes}          % mathop
\newcommand{\union}{\cup}                    % mathbin
\newcommand{\bigunion}{\bigcup}              % mathop
\newcommand{\intersect}{\cap}                % mathbin
\newcommand{\bigintersect}{\bigcap}          % mathop

\newcommand{\comp}{\circ}                    % mathbin
\newcommand{\cross}{\times}                  % mathbin

\newcommand{\isom}{\cong}                    % mathrel
\newcommand{\qisom}{\simeq}                  % mathrel
\newcommand{\nisom}{\ncong}                  % mathrel
\newcommand{\nqisom}{\not\simeq}             % mathrel
\newcommand{\superset}{\supset}              % mathrel
\newcommand{\contains}{\ni}                  % mathrel

% Special sets
\newcommand{\numset}[1]{\mathbb{#1}}
\newcommand{\N}{\numset{N}}
\newcommand{\Z}{\numset{Z}}
\newcommand{\Zpos}{\Z_{\geq 0}}
\newcommand{\Q}{\numset{Q}}
\newcommand{\R}{\numset{R}}
\newcommand{\C}{\numset{C}}
\newcommand{\F}[1]{\numset{F}_{#1}}
\newcommand{\cycgrp}[1]{\Z / #1 \Z}
\newcommand{\field}[1]{\mathbf{#1}}
\renewcommand{\j}{\field{j}}
\renewcommand{\k}{\field{k}}

% Punctuation
%\newcommand{\co}{\colon}
%\newcommand{\semico}{;\penalty 300}
\newcommand{\scolon}{; \penalty 300}

% Common operators
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\Id}{Id}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\Ker}{Ker}
\DeclareMathOperator{\Coker}{Coker}
\DeclareMathOperator{\im}{Im} % Image
\renewcommand{\Im}{\im}
\DeclareMathOperator{\homgy}{H} % Homology
\DeclareMathOperator{\Hom}{Hom} % Homomorphism
\DeclareMathOperator{\Cone}{Cone}
\DeclareMathOperator{\rk}{rk} % Rank
\DeclareMathOperator{\Hochsch}{HH} % Hochschild homology
\newcommand{\MCG}{\mathit{MCG}} % Mapping class group
\DeclareMathOperator{\Neg}{neg}


% Dodecahedral group
\newcommand{\Dod}{\mathrm{Dod}}

% Matrix groups
\newcommand{\matrixgrp}[1]{\mathrm{#1}}
\newcommand{\GL}{\matrixgrp{GL}}
\newcommand{\SL}{\matrixgrp{SL}}
\newcommand{\SO}{\matrixgrp{SO}}
\newcommand{\SU}{\matrixgrp{SU}}
\newcommand{\Sp}{\matrixgrp{Sp}}
\newcommand{\ISO}{\matrixgrp{ISO}}


% Lie algebras
\newcommand{\fsl}{\mathfrak{sl}}
\newcommand{\sltwo}{\fsl_2}
\newcommand{\fg}{\mathfrak g}
\newcommand{\fgl}{\mathfrak{gl}}
\newcommand{\gloneone}{\fgl_{1|1}}

% Basic topology
\newcommand{\torus}{\mathbb{T}}
\newcommand{\bdy}{\partial} % mathord
\newcommand{\connsum}{\mathbin{\#}} % Originally mathord
\newcommand{\bigconnsum}{\mathop{\mathchoice%
    {\vcenter{\hbox{\LARGE $\#$}}}
    {\vcenter{\hbox{\large $\#$}}}
    {\vcenter{\hbox{\footnotesize $\#$}}}
    {\vcenter{\hbox{\scriptsize $\#$}}}
  }}
\newcommand{\bdysum}{\mathbin{\natural}} % Originally mathord
\newcommand{\bigbdysum}{\mathop{\mathchoice%
    {\vcenter{\hbox{\LARGE $\natural$}}}
    {\vcenter{\hbox{\large $\natural$}}}
    {\vcenter{\hbox{\footnotesize $\natural$}}}
    {\vcenter{\hbox{\scriptsize $\natural$}}}
  }}
\DeclareMathOperator{\Sym}{Sym}
\newcommand{\unknot}{\mathord{\bigcirc}} % Originally mathbin
\newcommand{\quasialt}{\mathcal{Q}} % Quasi-alternating links
\newcommand{\QHS}{{\Q}\mathit{HS}^3}
\newcommand{\ZHS}{{\Z}\mathit{HS}^3}
\newcommand{\nbhd}[1]{\nu (#1)}

% interior of a subspace
\DeclareMathOperator{\interior}{int}


% Spheres, disks, ...
\newcommand{\sphere}[1]{\mathbb{S}^{#1}}
\newcommand{\disk}[1]{\mathbb{D}^{#1}}
\newcommand{\ball}[1]{\mathbb{B}^{#1}}
\newcommand{\interval}{\mathbb{I}}
\newcommand{\RP}[1]{\mathbb{RP}^{#1}}
\newcommand{\CP}[1]{\mathbb{CP}^{#1}}

% Point
\newcommand{\point}{\textup{pt}}

\newcommand{\laurent}{\ZZ[t, t^{-1}]}
% Blanchfield
\newcommand{\Bl}{\operatorname{Bl}}

% Shortcuts for blackboard letters
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\HH}{\mathbb{H}}

% Free groups
\DeclareMathOperator{\Fr}{Fr}

% (Twist) spinning knots
\newcommand{\Spin}{\tau}

% topological, smooth category
\newcommand{\topological}{\mathrm{top}}
\newcommand{\sm}{\mathrm{sm}}

% Untwisting number
\DeclareMathOperator{\tu}{tu}
% Surgery description number
\DeclareMathOperator{\sd}{sd}
% algebraic genus
\newcommand{\alggenus}{g_{\mathrm{alg}}}
